Grounded Keys-to-Text Generation: Towards Factual Open-Ended Generation

Large pre-trained language models have recently enabled open-ended generation frameworks (e.g., prompt-to-text NLG) to tackle a variety of tasks going beyond the traditional data-to-text generation. While this framework is more general, it is under-specified and often leads to a lack of controllability restricting their real-world usage. We propose a new grounded keys-to-text generation task: the task is to generate a factual description about an entity given a set of guiding keys, and grounding passages. To address this task, we introduce a new dataset, called EntDeGen. Inspired by recent QA-based evaluation measures, we propose an automatic metric, MAFE, for factual correctness of generated descriptions. Our EntDescriptor model is equipped with strong rankers to fetch helpful passages and generate entity descriptions. Experimental result shows a good correlation (60.14) between our proposed metric and human judgments of factuality. Our rankers significantly improved the factual correctness of generated descriptions (15.95% and 34.51% relative gains in recall and precision). Finally, our ablation study highlights the benefit of combining keys and groundings.

==> tables/QA_metric_res.tex <==
% \setlength\tabcolsep{3.5pt}
% \renewcommand{\arraystretch}{1.6}
% \begin{tabular}{l|l|ccc}
% \hline
% \textbf{Model}                     & \textbf{Ranker}& \textbf{Int. Precision} & \textbf{Recall} & \textbf{Ext. Precision} \\ \hline
% \multirow{5}{*}{\textbf{T5-Large}} & Unranked       & 16.15 & 17.66 &   \\
%                                   & Tf-idf         &  &  &   \\
%                                   & Contrastive Dense    & 18.28  & 19.00 &   \\
%                                   & Autoregressive &    18.74   &   \textbf{19.48}    &      \\ \cdashline{2-5} 
%                                   & \textit{Rouge2 (oracle)}         &    20.48  &    20.99   &    51.82   \\ \hline
% \multirow{5}{*}{\textbf{BART-L}}   & Unranked       &  22.04 & 17.43 &   34.88   \\
%                                   & Tf-idf         &  22.82 &  17.45 &      35.88\\
%                                   & Contrastive Dense    &  24.71  &  18.55 &  42.68  \\
%                                   & Autoregressive &   \textbf{25.63}   &  19.11  &  42.52  \\ \cdashline{2-5} 
%                                   & \textit{Rouge2 (oracle)}       &   27.99  &   20.28    &   40.90   \\ \hline
% \multirow{5}{*}{\textbf{PEGASUS}}  & Unranked       & 20.15 & 15.34 &  \\
%                                   & Tf-idf         &       &       &        \\
%                                   & Contrastive Dense    & 22.17  & 16.40 &  \\
%                                   & Autoregressive &  22.51   &   17.16  &   46.77   \\ \cdashline{2-5} 
%                                   & \textit{Rouge2 (oracle)}         &    23.90     &   18.07  &   43.84  \\ \hline
% \end{tabular}


\setlength\tabcolsep{3.5pt}
\renewcommand{\arraystretch}{1.6}
\begin{tabular}{l|l|ccc}
\hline
\textbf{Model}                     & \textbf{Ranker}& \textbf{Recall} & \textbf{Int. Precision} & \textbf{Ext. Precision} \\ \hline
\multirow{5}{*}{\textbf{T5-Large}} & Unranked       &  17.66 &  16.15 & \\
                                   & Tf-idf         &  &  &   \\
                                   & Contrastive Dense    &  19.00 &   18.28  & \\
                                   & Autoregressive &    \textbf{19.48}    &    18.74   &     \\ \cdashline{2-5} 
                                   & \textit{Rouge2 (oracle)}         &    20.99   &   20.48  &     51.82   \\ \hline
\multirow{5}{*}{\textbf{BART-L}}   & Unranked       &  17.43 &   22.04 & 34.88   \\
                                   & Tf-idf         & 17.45 &    22.82 &      35.88\\
                                   & Contrastive Dense    &   18.55 & 24.71  &  42.68  \\
                                   & Autoregressive &    19.11  & \textbf{25.63}   &  42.52  \\ \cdashline{2-5} 
                                   & \textit{Rouge2 (oracle)}       &     20.28    & 27.99  &   40.90   \\ \hline
\multirow{5}{*}{\textbf{PEGASUS}}  & Unranked       & 15.34 &  20.15 &  \\
                                   & Tf-idf         &       &       &        \\
                                   & Contrastive Dense    & 16.40 &  22.17  &  \\
                                   & Autoregressive &    17.16  &  22.51   &  46.77   \\ \cdashline{2-5} 
                                   & \textit{Rouge2 (oracle)}         &     18.07  &   23.90     &  43.84  \\ \hline
\end{tabular}


% \setlength\tabcolsep{3.5pt}
% \renewcommand{\arraystretch}{1.6}
% \begin{tabular}{l|l|ccc}
% \hline
% \textbf{Model}                     & \textbf{Ranker}& \textbf{Int. Precision} & \textbf{Recall} & \textbf{Ext. Precision} \\ \hline
% \multirow{5}{*}{\textbf{T5-Large}} & Unranked       & 16.15 & 7.65 &   \\
%                                   & Tf-idf         &  &  &   \\
%                                   & Contrastive Dense    & 18.28  & 9.25 &   \\
%                                   & Autoregressive &    18.74   &   9.45    &      \\ \cdashline{2-5} 
%                                   & \textit{Rouge2 (oracle)}         &    20.48  &    10.45   &    51.82   \\ \hline
% \multirow{5}{*}{\textbf{BART-L}}   & Unranked       &  22.04 & 17.43 &   34.88   \\
%                                   & Tf-idf         &  22.82 &  17.45 &      35.88\\
%                                   & Contrastive Dense    &  24.71  &  18.55 &  42.68  \\
%                                   & Autoregressive &   \textbf{25.63}   &  \textbf{19.11}   &  42.52  \\ \cdashline{2-5} 
%                                   & \textit{Rouge2 (oracle)}       &   27.99  &   20.28    &   40.90   \\ \hline
% \multirow{5}{*}{\textbf{PEGASUS}}  & Unranked       & 20.15 & &  \\
%                                   & Tf-idf         &       &       &        \\
%                                   & Contrastive Dense    & 22.17  & 8.06 &  \\
%                                   & Autoregressive &  22.51   &   8.38  &   46.77   \\ \cdashline{2-5} 
%                                   & \textit{Rouge2 (oracle)}         &    23.90     &   9.10  &   43.84  \\ \hline
% \end{tabular}

==> tables/all_auto_res.tex <==


% Please add the following required packages to your document preamble:
% \usepackage{multirow}

\renewcommand{\arraystretch}{1.4}
\begin{tabular}{l|l|llll}
\hline
\textbf{Model}                     & \textbf{Ranker}         & \textbf{BLEU} & \textbf{R-1} & \textbf{R-2} & \textbf{R-L} \\ \hline
\multirow{5}{*}{\textbf{T5-Large}} & Unranked       &   5.41   &   28.74  &   10.31  &  26.08   \\
                          & Tf-idf  &  5.50    &    29.49  &   10.54  &  26.70  \\
                          & Cont. Dense    &   6.89   &   30.92  &  12.19   &  28.14   \\
                          & Autoregressive   &    7.24  &   31.45  &  12.59   &   28.64  \\ \cdashline{2-6}
                          & \textit{Rouge2 (cheat})       &  8.56    &  33.75   &   14.84  &   30.84  \\ \hline 
\multirow{5}{*}{\textbf{BART-L}}   & Unranked       &   7.03   &  33.52   &  14.39  &   30.82  \\
                          & Tf-idf         &   6.97   &  34.00   &   14.54  &  31.14   \\
                          & Cont. Dense    &   8.25   &  35.26   &  16.04   &   32.46  \\
                          & Autoregressive &   \textbf{8.69}   &   \textbf{35.80}  &  \textbf{16.62}   &   \textbf{32.97}  \\ \cdashline{2-6}
                          & \textit{Rouge2 (cheat)}   &  9.82    &   37.72   &   18.57  &  34.87  \\ \hline
\multirow{5}{*}{\textbf{PEGASUS}}  & Unranked       &   6.49   &  29.23   &  12.46   &   27.11  \\
                          & Tf-idf         &      &     &     &     \\
                          & Cont. Dense    &   7.99   &  31.21   &  14.16   &   28.94  \\
                          & Autoregressive &   8.55   &  32.03   &  14.90   &  29.75   \\ \cdashline{2-6}
                          & \textit{Rouge2 (cheat)}         &   10.05   &   34.01  &  17.03   &   31.71  \\ \hline
\end{tabular}


==> tables/all_auto_res_2.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}

%%% earlier version with R-1 R-2 and Par-p, and Par-R 
% \setlength\tabcolsep{6pt}
% \renewcommand{\arraystretch}{1.5}
% \begin{tabular}{l|l|cccc|ccc|c}
% \hline
% \textbf{Model}                     & \textbf{Ranker}         & \textbf{BLEU} & \textbf{R-1} & \textbf{R-2} & \textbf{R-L} & \textbf{PAR-P} & \textbf{PAR-R} & \textbf{PAR-F1} & \textbf{BERTScore}\\ \hline
% \textbf{Extractive-QA}             & n/a        &    2.94    &    22.37    &     6.28     &    19.85     &   43.17  &  10.45   &  14.22  & 82.44 \\ \hline
% \multirow{5}{*}{\textbf{T5-Large}} & Unranked                &        5.41       &       28.74       &       10.31       &       26.8       &        51.89    &    15.09   &    20.58  & 84.25\\
%                                   & Tf-idf    &          5.50    &    29.49  &   10.54  &  26.70       &     52.88   &  15.73   &    21.42  & 84.53 \\
%                                   & Contrastive Dense             &         6.89   &   30.92  &  12.19   &  28.14      &   50.66    &    16.91   &     22.44 & 84.92 \\
%                                   & Autoregressive          &     7.24  &   31.45  &  12.59   &   28.64      &    52.10   &   17.66    &    23.45   & 84.96 \\ \cdashline{2-10} 
%                                   & \textit{Rouge2 (oracle)} &         8.56    &  33.75   &   14.84  &   30.84         &    54.12   &    19.77   &     25.97  & 85.41 \\ \hline
% \multirow{5}{*}{\textbf{BART-L}}   & Unranked                &        7.03   &  33.52   &  14.39  &   30.82      &   60.23    &    16.85   & 23.57   & 86.10    \\
%                                   & Tf-idf                  &         6.97   &  34.00   &   14.54  &  31.14      &   59.91    &    17.06   &    23.96  & 86.23 \\
%                                   & Contrastive Dense             &       8.25   &  35.26   &  16.04   &   32.46    &    58.19   &    17.91   &    24.67  & 86.48  \\
%                                   & Autoregressive          &       \textbf{8.69}   &   \textbf{35.80}  &  \textbf{16.62}   &   \textbf{32.97}    &    59.29   &    18.47   &    \textbf{25.40}  & \textbf{86.58}  \\ \cdashline{2-10} 
%                                   & \textit{Rouge2 (oracle)} &       9.82    &   37.72   &   18.57  &  34.87    &    60.82   &   19.93    &    27.25   & 87.01 \\ \hline
% \multirow{5}{*}{\textbf{PEGASUS}}  & Unranked                &           6.49   &  29.23   &  12.46   &   27.11         &   \textbf{66.67}    &    16.45   &    22.88  & 83.65  \\
%                                   & Tf-idf                  &         6.34      &       29.43       &      12.38        &       27.25       &       65.11         &      16.16          &         22.68    &  83.74  \\
%                                   & Contrastive Dense             &         7.99   &  31.21   &  14.16   &   28.94       &    62.44   &   17.70    &     24.10  & 84.43 \\
%                                   & Autoregressive          &       8.55   &  32.03   &  14.90   &  29.75     &   64.04    &    \textbf{18.74}   &     25.38  & 84.54 \\ \cdashline{2-10} 
%                                   & \textit{Rouge2 (oracle)} &           10.05   &   34.01  &  17.03   &   31.71         &    65.69     &    20.61   &    27.72  & 84.97  \\ \hline
% \end{tabular}
% \setlength\tabcolsep{8pt}



%%% correct precision
\setlength\tabcolsep{4.5pt}
\renewcommand{\arraystretch}{1.5}
\begin{tabular}{l|l|cc|c|c|cc}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Ranker}} & \multirow{2}{*}{\textbf{BLEU}} & \multirow{2}{*}{\textbf{R-L}} & \multirow{2}{*}{\textbf{PARENT}} & \multirow{2}{*}{\textbf{BERT-S}} & \multicolumn{2}{c}{\textbf{MAFE}}               \\ \cline{7-8} 
                      &                                  &                                &                                   &                               &                                     & Recall & Precision\\ \hline
\textbf{Extractive}             & n/a        &    2.94      &    19.85     &   14.22  & 82.44 & 19.01 & 18.91  \\ \hline
\multirow{5}{*}{\textbf{T5-Large}} & Unranked                &        5.41     &     15.09   &    20.58  & 84.25  &  17.65 &  17.38 \\
                                  & Tf-idf    &          5.50    &  26.70       &   21.42  & 84.53 & 17.68 & 18.35  \\
                                  & Contrastive Dense             &         6.89   &  28.14  &     22.44 & 84.92   &  19.00 &   19.66 \\
                                  & Autoregressive          &     7.24  &   28.64      &   23.45   & 84.96 & \textbf{19.48}    &    19.97    \\ \cdashline{2-8} 
                                  & \textit{Rouge2 (oracle)} &         8.56    &  30.84   &     25.97  & 85.41   &    20.99   &   22.01   \\ \hline
\multirow{5}{*}{\textbf{BART-L}}   & Unranked                &        7.03   &  30.82    & 23.57   & 86.10  &  17.43 &   23.13  \\
                                  & Tf-idf                  &         6.97   &   31.14    &    23.96  & 86.23   & 17.45 &    24.02    \\
                                  & Contrastive Dense             &       8.25  &   32.46    &    24.67  & 86.48    &   18.55 & 26.00  \\
                                  & Autoregressive          &       \textbf{8.69}   &    \textbf{32.97}    &   \textbf{25.40}  & \textbf{86.58}  &    19.11  & \textbf{26.71}   \\ \cdashline{2-8} 
                                  & \textit{Rouge2 (oracle)} &       9.82    &  34.87    &     27.25   & 87.01   &     20.28    & 29.32  \\ \hline
\multirow{5}{*}{\textbf{PEGASUS}}  & Unranked                &           6.49  &   27.11         &    22.88  & 83.65     & 15.34 &  22.72 \\
                                  & Tf-idf                  &         6.34   &       27.25     &         22.68    &  83.74  & 14.79 &  23.72 \\
                                  & Contrastive Dense     &         7.99   &   28.94     &     24.10  & 84.43 & 16.40 &  24.70  \\
                                  & Autoregressive          &       8.55   &   29.75     &  25.38  & 84.54 &    17.16  &  25.34   \\ \cdashline{2-8} 
                                  & \textit{Rouge2 (oracle)} &           10.05   &    31.71   &    27.72  & 84.97  &     18.07  &   26.73    \\ \bottomrule
\end{tabular}
\setlength\tabcolsep{8pt}



% %%% correct precision / with faithfulness on 40
% \setlength\tabcolsep{4.5pt}
% \renewcommand{\arraystretch}{1.5}
% \begin{tabular}{l|l|cc|c|c|ccc}
% \toprule
% \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Ranker}} & \multirow{2}{*}{\textbf{BLEU}} & \multirow{2}{*}{\textbf{R-L}} & \multirow{2}{*}{\textbf{PARENT}} & \multirow{2}{*}{\textbf{BERT-S}} & \multicolumn{3}{c}{\textbf{MAFE}}               \\ \cline{7-9} 
%                       &                                  &                                &                                   &                               &                                     & Recall & Precision (Int.) & Precision (Ext.) \\ \hline
% \textbf{Extractive-QA}             & n/a        &    2.94      &    19.85     &   14.22  & 82.44 & 19.01 & 18.91 & \\ \hline
% \multirow{5}{*}{\textbf{T5-Large}} & Unranked                &        5.41     &     15.09   &    20.58  & 84.25  &  17.65 &  17.38 & \\
%                                   & Tf-idf    &          5.50    &  26.70       &   21.42  & 84.53 & 17.68 & 18.35 & \\
%                                   & Contrastive Dense             &         6.89   &  28.14  &     22.44 & 84.92   &  19.00 &   19.66  & \\
%                                   & Autoregressive          &     7.24  &   28.64      &   23.45   & 84.96 & \textbf{19.48}    &    19.97   &     \\ \cdashline{2-9} 
%                                   & \textit{Rouge2 (oracle)} &         8.56    &  30.84   &     25.97  & 85.41   &    20.99   &   22.01  &      \\ \hline
% \multirow{5}{*}{\textbf{BART-L}}   & Unranked                &        7.03   &  30.82    & 23.57   & 86.10  &  17.43 &   23.13 &   \\
%                                   & Tf-idf                  &         6.97   &   31.14    &    23.96  & 86.23   & 17.45 &    24.02 &       \\
%                                   & Contrastive Dense             &       8.25  &   32.46    &    24.67  & 86.48    &   18.55 & 26.00  &  \\
%                                   & Autoregressive          &       \textbf{8.69}   &    \textbf{32.97}    &   \textbf{25.40}  & \textbf{86.58}  &    19.11  & \textbf{26.71}   &  39.10\\ \cdashline{2-9} 
%                                   & \textit{Rouge2 (oracle)} &       9.82    &  34.87    &     27.25   & 87.01   &     20.28    & 29.32  &   37.52 \\ \hline
% \multirow{5}{*}{\textbf{PEGASUS}}  & Unranked                &           6.49  &   27.11         &    22.88  & 83.65     & 15.34 &  22.72 & \\
%                                   & Tf-idf                  &         6.34   &       27.25     &         22.68    &  83.74  & 14.79 & & \\
%                                   & Contrastive Dense             &         7.99   &   28.94     &     24.10  & 84.43 & 16.40 &  24.70  & \\
%                                   & Autoregressive          &       8.55   &   29.75     &  25.38  & 84.54 &    17.16  &  25.34   &   \\ \cdashline{2-9} 
%                                   & \textit{Rouge2 (oracle)} &           10.05   &    31.71   &    27.72  & 84.97  &     18.07  &   26.73     &   \\ \toprule
% \end{tabular}
% \setlength\tabcolsep{8pt}

%%% Older version - mafe precision differently / faithfulness on top-10 groudnings
% \setlength\tabcolsep{4.5pt}
% \renewcommand{\arraystretch}{1.5}
% \begin{tabular}{l|l|cc|c|c|ccc}
% \hline
% \multirow{2}{*}{Model} & \multirow{2}{*}{\textbf{Ranker}} & \multirow{2}{*}{\textbf{BLEU}} & \multirow{2}{*}{\textbf{R-L}} & \multirow{2}{*}{\textbf{PARENT}} & \multirow{2}{*}{\textbf{BERT-S}} & \multicolumn{3}{c}{\textbf{MAFE}}               \\ \cline{7-9} 
%                       &                                  &                                &                                   &                               &                                     & Recall & Precision (Int.) & Precision (Ext.) \\ \hline
% \textbf{Extractive-QA}             & n/a        &    2.94      &    19.85     &   14.22  & 82.44 & & & \\ \hline
% \multirow{5}{*}{\textbf{T5-Large}} & Unranked                &        5.41     &     15.09   &    20.58  & 84.25  &  17.65 &  16.15 & \\
%                                   & Tf-idf    &          5.50    &  26.70       &   21.42  & 84.53 & 17.68 & 16.99 & 49.61\\
%                                   & Contrastive Dense             &         6.89   &  28.14  &     22.44 & 84.92   &  19.00 &   18.28  & \\
%                                   & Autoregressive          &     7.24  &   28.64      &   23.45   & 84.96 & \textbf{19.48}    &    18.74   &     \\ \cdashline{2-9} 
%                                   & \textit{Rouge2 (oracle)} &         8.56    &  30.84   &     25.97  & 85.41   &    20.99   &   20.48  &     51.82 \\ \hline
% \multirow{5}{*}{\textbf{BART-L}}   & Unranked                &        7.03   &  30.82    & 23.57   & 86.10  &  17.43 &   22.04 & 34.88  \\
%                                   & Tf-idf                  &         6.97   &   31.14    &    23.96  & 86.23   & 17.45 &    22.82 &      35.88 \\
%                                   & Contrastive Dense             &       8.25  &   32.46    &    24.67  & 86.48    &   18.55 & 24.71  &  42.68 \\
%                                   & Autoregressive          &       \textbf{8.69}   &    \textbf{32.97}    &   \textbf{25.40}  & \textbf{86.58}  &    19.11  & \textbf{25.63}   &  42.52\\ \cdashline{2-9} 
%                                   & \textit{Rouge2 (oracle)} &       9.82    &  34.87    &     27.25   & 87.01   &     20.28    & 27.99  &   40.90 \\ \hline
% \multirow{5}{*}{\textbf{PEGASUS}}  & Unranked                &           6.49  &   27.11         &    22.88  & 83.65     & 15.34 &  20.15 & \\
%                                   & Tf-idf                  &         6.34   &       27.25     &         22.68    &  83.74  & 14.79 & & \\
%                                   & Contrastive Dense             &         7.99   &   28.94     &     24.10  & 84.43 & 16.40 &  22.17  & \\
%                                   & Autoregressive          &       8.55   &   29.75     &  25.38  & 84.54 &    17.16  &  22.51   &  46.77  \\ \cdashline{2-9} 
%                                   & \textit{Rouge2 (oracle)} &           10.05   &    31.71   &    27.72  & 84.97  &     18.07  &   23.90     &  43.84 \\ \hline
% \end{tabular}
% \setlength\tabcolsep{8pt}

==> tables/n-gram-results.tex <==
\setlength\tabcolsep{6pt}
    \renewcommand{\arraystretch}{1.1}
    \begin{tabular}{lcccc}
    \toprule
    \textbf{Model} & \textbf{BLEU} & \textbf{R-1} & \textbf{R-2} & \textbf{R-L} \\ 
    \midrule
    GPT2-M & & & & \\
    T5-Large & 8.56 & 33.75 & 14.84 & 30.84 \\
    BART-L & 9.82 & 37.72 & 18.57 & 34.87\\
    PEGASUS & 10.05 & 34.01 & 17.03 & 31.71\\
    \bottomrule
    \end{tabular}
\setlength\tabcolsep{6pt}

==> tables/parent-res.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\renewcommand{\arraystretch}{1.4}
\begin{tabular}{l|l|lll}
\hline
\textbf{Model}                     & \textbf{Ranker}& \textbf{PAR-P} & \textbf{PAR-R} & \textbf{PAR-F1} \\ \hline
\multirow{5}{*}{\textbf{T5-Large}} & Unranked       &   51.89    &    15.09   &    20.58    \\
                                   & Tf-idf         &    52.88   &  15.73   &    21.42  \\
                                   & Cont. Dense    &   50.66    &    16.91   &     22.44   \\
                                   & Autoregressive &    52.10   &   17.66    &    23.45    \\ \cdashline{2-5} 
                                   & \textit{Rouge2 (cheat)}         &    54.12   &    19.77   &     25.97   \\ \hline
\multirow{5}{*}{\textbf{BART-L}}   & Unranked       &   60.23    &    16.85   & 23.57       \\
                                   & Tf-idf         &   59.91    &    17.06   &    23.96    \\
                                   & Cont. Dense    &    58.19   &    17.91   &    24.67    \\
                                   & Autoregressive &    59.29   &    18.47   &    \textbf{25.40}    \\ \cdashline{2-5} 
                                   & \textit{Rouge2 (cheat)}         &    60.82   &   19.93    &    27.25    \\ \hline
\multirow{5}{*}{\textbf{PEGASUS}}  & Unranked       &   \textbf{66.67}    &    16.45   &    22.88    \\
                                   & Tf-idf         &       &       &        \\
                                   & Cont. Dense    &    62.44   &   17.70    &     24.10  \\
                                   & Autoregressive &   64.04    &    \textbf{18.74}   &     25.38   \\ \cdashline{2-5} 
                                   & \textit{Rouge2 (cheat)}         &    65.69     &    20.61   &    27.72    \\ \hline
\end{tabular}


